Rigidity for infinitely renormalizable area-preserving maps

The period doubling Cantor sets of strongly dissipative Henon-like maps with different average Jacobian are not smoothly conjugated. The Jacobian Rigidity Conjecture says that the period doubling Cantor sets of two-dimensional Henon-like maps with the same average Jacobian are smoothly conjugated. This conjecture is true for average Jacobian zero, e.g. the one-dimensional case. The other extreme case is when the maps preserve area, e.g. the average Jacobian is one. Indeed, the period doubling Cantor set of area-preserving maps in the universality class of the Eckmann-Koch-Wittwer renormalization fixed point are smoothly conjugated.

==> dynamics.tex <==
\section{Dynamics on the Cantor set}\label{dynamics}

==> prelimIII.tex <==

\section{Preliminaries}\label{prelim}

A complete discussion of the following definitions and statements can be found in part I and part II, see \cite{CLM}, \cite{LM1}, of this series on renormalization of H\'enon-like maps.

\bigskip

Let $\Omega^h, \Omega^v\subset \mathbb{C}$ be neighborhoods of $[-1,1]\subset \mathbb{R}$ and $\Omega=\Omega^h\times \Omega^v$.  The set
 $\HH_\Omega(\overline{\epsilon})$ consists of maps $F:[-1,1]^2\to [-1,1]^2$ of the following form.
$$
F(x,y)=(f(x)-\epsilon(x,y), x),
$$
where $f:[-1,1]\to [-1,1]$ is a unimodal map which admits a holomorphic extension to $\Omega^h$ and $\epsilon:[-1,1]^2\to \mathbb{R}$ admits  a holomorphic extension to $\Omega$ and finally, $|\epsilon|\le \overline{\epsilon}$. The critical point $c$ of $f$ is non degenerate, $D^2f(c)<0$. A map in  $\HH_\Omega(\overline{\epsilon})$ is called a {\it H\'enon-like} map. Observe that H\'enon-like maps map vertical lines to horizontal lines.


A unimodal map $f:[-1,1]\to [-1,1]$ with critical point $c\in [-1,1]$ is {\it renormalizable} if $f^2:[f^2(c),f^4(c)]\to [f^2(c),f^4(c)]$ is unimodal and 
$[f^2(c),f^4(c)]\cap f([f^2(c),f^4(c)])=\emptyset$. The renormalization of $f$ 
is the affine rescaling of $f^2|([f^2(c),f^4(c)]$, denoted by $Rf$. The domain of $Rf$ is again $[-1,1]$.  The renormalization operator $R$ has a unique fixed 
point $f_*:[-1,1]\to [-1,1]$.  The introduction of \cite{FMP} presents the history of renormalization of unimodal maps and describes the main results.

The {\it scaling factor} of this fixed point $f_*$ is
$$
\sigma=\frac{|[f_*^2(c),f_*^4(c)]|}{|[-1,1]|}.
$$  


A H\'enon-like map is renormalizable if there exists a domain $D\subset [-1,1]^2$ such that
$F^2:D\to D$. The construction of the domain $D$ is inspired by renormalization of unimodal maps. In particular, it should be a topological construction.  However, for small $\overline{\epsilon}>0$ the actual domain $A\subset [-1,1]$, used to renormalize as was done in \cite{CLM}, has an analytical definition. The precise definition can be found in \S 3.5 of part I. If the renormalizable H\'enon-like maps is given by  $F(x,y)=(f(x)-\epsilon(x,y))$ then the 
domain $A\subset [-1,1]$, an essentially vertical strip, is bounded by two curves of the form 
$$
f(x)-\epsilon(x,y)=\text{Const}.
$$
These curves are graphs over the $y$-axis with a slope of the order 
$\overline{\epsilon}>0$. 
The domain $A$ satisfies similar combinatorial properties as the domain of renormalization of a unimodal map:
$$
F(A)\cap A=\emptyset,
$$
and
$$
F^2(A)\subset A.
$$
Unfortunately, the restriction $F^2|A$ is not a H\'enon-like map 
as it does not map vertical lines into horizontal lines. 
This is the reason why the coordinated change needed to define the renormalization of $F$ is not an affine map, 
but it rather has the following form. Let
$$
H(x,y)=(f(x))-\epsilon(x,y),y)
$$
and
$$
G=H\circ F^2\circ H^{-1}.
$$
The map $H$ preserves horizontal lines and it is designed in such a way
 that the map $G$ maps vertical lines into horizontal lines. 
Moreover, $G$ is well defined on a rectangle $U\times [-1, 1]$ of 
full height. Here $U\subset [-1,1]$ is an interval of length $2/|s|$ 
with $s<-1$. 
Let us  rescale the domain of $G$ by the $s$-dilation $\Lambda$, 
such that the rescaled domain is of the form $[-1,1]\times V$,
where $V\subset \mathbb{R}$ is an interval of length $2/|s|$. Define the renormalization of $F$ by
$$
RF= \Lambda\circ G\circ \Lambda^{-1}.
$$
Notice that $RF$ is well defined on the rectangle $[-1,1]\times V$.
The coordinate  change $\psi= H^{-1}\circ \La^{-1}$ maps this rectangle 
onto the
topological rectangle  $A$ of full height.  


The set of $n$-times renormalizable maps is denoted by $\HH^n_\Omega(\overline{\epsilon})\subset \HH_\Omega(\overline{\epsilon})$. If 
$F\in \HH^n_\Omega(\overline{\epsilon})$ we 
use the notation
$$
F_n=R^nF.
$$
The set of infinitely renormalizable maps is denoted by
$$
\II_\Omega(\overline{\epsilon})=\bigcap_{n\ge 1} 
\HH^n_\Omega(\overline{\epsilon}).
$$


The renormalization operator acting on $\HH^1_\Omega(\overline{\epsilon})$,
$\overline{\epsilon}>0$ small enough, has a unique fixed point
 $F_*\in \II_\Omega(\overline{\epsilon})$. It is the degenerate map 
$$
F_*(x,y)=(f_*(x), x).
$$
This renormalization fixed point is hyperbolic and the stable manifold has codimension one. Moreover,
$$
W^s(F_*)=\II_\Omega(\overline{\epsilon}).
$$

If we want to emphasize that some set, say $A$, 
is associated with a certain map $F$ we 
use notation like $A(F)$.

The coordinate change which conjugates $F_k^2|A(F_k)$ to $F_{k+1}$ is
 denoted 
by
\begin{equation}\label{phi}
          \psi^{k+1}_v=(\Lambda_k \circ H_k)^{-1}: \Domain(F_{k+1})\to A(F_k). 
\end{equation}
Here $H_k$ is the non-affine part of the coordinate change used to define 
$R^{k+1}F$ and $\Lambda_k$ is the dilation by $s_k<-1$.
Now, for $k<n$, let
\begin{equation}\label{Phi}
\Psi^n_k=\psi^{k+1}_v\circ \psi^{k+2}_v\circ \cdots \circ \psi^{n}_v:
\Domain(F_{n})\to A_{n-k}(F_k),
\end{equation}
where
$$
A_k(F)=\Psi^k_0(\Domain(F_k))\cap B.
$$
Notice, that each $A_k\subset [-1,1]$ is of full height and 
$\Psi^k_0$ conjugates $R^kF$ to $F^{2^k}|A_k$.
Furthermore,
$
A_{k+1}\subset A_k
$.

\bigskip



The change of
coordinates conjugating the renormalization $RF$ to $F^2$ is denoted by
  $\psi_v^1 := H^{-1}\circ \La^{-1}$. To describe the attractor of an infinitely renormalizable H\'enon-like map we also need the map $\psi_c^1= F\circ
\psi^1_v$. The subscripts $v$ and $c$ indicate that these maps are
associated to the critical {\it value} and the {\it critical} point,
respectively.


Similarly, let $\psi^2_v$ and $\psi^2_c$ be the corresponding
changes of variable for $RF$, and let
$$
\psi^2_{vv}= \psi^1_v\circ \psi^2_v, \quad \psi^2_{cv}= \psi^1_c\circ
\psi^2_v, \quad \psi^2_{vc}=\psi^1_v\circ\psi^2_c,\quad \psi^2_{cc}=\psi^1_c\circ \psi^2_c.
$$
and, proceeding this way, for any $n\ge 0$, construct $2^{n}$ maps 
$$ \psi^n_w = \psi^1_{w_1}\circ\dots\circ \psi^n_{w_{n}}, \quad
w=(w_1, \dots, w_{n})\in\{v,c\}^{n}. $$ 
The notation $\psi^n_w(F)$ will also be used to emphasize the map
under consideration, and we will let $W=\{v,c\}$ and
$W^n=\{v,c\}^n$ be the $n$-fold Cartesian product. The following Lemma and its proof can be found in \cite[Lemma 5.1]{CLM}.


\begin{lem}\label{contracting}
Let $F\in \II^c_\Om(\bar\eps)$. There exist $C>0$ 
such that for  $w\in W^n$, 
$
\| D\psi^n_w\|\leq  C \sigma^n,
$
$n\ge 1$.
\end{lem}

Let  $F\in \II_\Omega(\overline{\epsilon})$ and consider the domains
$$
B^n_\omega=\Im \psi^n_\omega.
$$
The first return maps to the domains
$$
B^n_{v^n}=\Im \Psi^n_0=\Im \psi^n_{v^n}
$$
correspond to the different renormalizations.
Notice, 
$$
B^{n+1}_{v^{n+1}}\subset B^n_{v^n}.
$$
An infinitely renormalizable H\'enon-like  map has an invariant Cantor set:
$$
\OO_F=\bigcap_{n\ge 1} \bigcup_{i=0}^{2^n-1} F^i(B^n_{v^n})=
\bigcap_{n\ge 1} \bigcup_{\omega\in W^n} B^n_\omega.
$$ 
The dynamics on this Cantor set
 is conjugate to an adding machine. Its unique invariant measure is denoted 
by $\mu$. 
The {\it average  Jacobian}
$$
b_F=\exp\int \log \Jac F d\mu
$$ 
with respect to $\mu$ is an important parameter that
influences the geometry of $\OO_F$, see \cite[Theorem 10.1]{CLM}.  


The critical point (and critical value) of a unimodal map plays a crucial role 
in its dynamics. The counterpart of the critical value for infinitely renormalizable H\'enon-like maps is the 
{\it tip}
$$
\{\tau_F\}=\bigcap_{n\ge 1} B^n_{v^n}.
$$

\subsection{One-dimensional maps}\label{1D universal f-s} 
Recall that  $f_*\colon [-1,1] \to [-1,1]$ stands for the one-dimensional
renormalization fixed point % acting on its dynamical interval,
normalized so that $f_*(c_*)=1$ and $f_*^2(c_*)=-1$, where 
$c_*\in [-1,1]$ is the  critical point of $f_*$. 
\comment{
We let $J_c^* =[-1, f_*^4(c_*)]$ be the smallest renormalization interval of $f_*$, 
and   we let $s\colon J_c^*\ra  I$ be the orientation reversing affine rescaling.
The smallest renormalization interval around the critical value is denoted by
 $J_v^*= f_*(J^*_c)=[f_*^3(c_*),1]$.
Then $s\circ f_*: J_v^*\ra [-1,1] $ is an expanding  diffeomorphism.
Consider the inverse contraction  
\[
    g_*\colon [-1,1]\to J^*_v, \quad g_*=f_*^{-1}\circ s^{-1},
\]
where $f_*^{-1}$ stands for the branch of the inverse map that maps $J_c^*$ onto  $J_v^*$. 
The function $g_*$ is the non-affine branch of the so called ``presentation function''
(see~\cite{BMT} and references therein).
Note that $1$ is the unique fixed point of $g_*$.

 Let $J_c^*(n) \subset [-1,1]$ be the smallest periodic interval of period $2^n$ that contains $c_*$ and $J_v^*(n) \subset [-1,1]$ be the smallest periodic interval of period $2^n$ that contains $1$.

Let
$G_*^n\colon [-1,1]\to [-1,1]$ be the diffeomorphism obtained by rescaling
affinely the image of $g_*^n$. The fact that $g_*$ is a contraction implies
that the following limit exists 
\[
u_*=\lim_{n\to \infty} G_*^n \colon [-1,1]\to [-1,1],  
\]
where the convergence is exponential in the $C^3$-topology.
In fact, this function linearizes $g_*$ near the attracting fixed point $1$ 
(see, e.g., \cite[Theorem 8.2]{Mi}). The following Lemma and its proof can be found in \cite[Lemma 7.1]{CLM}.

\begin{lem} \label{ustarfstar} For every $n\ge 1$
\begin{enumerate}
\item [\rm (1)] $J^*_v(n)=g_*^n(I)$,

\item [\rm (2)] $R^n_vf_*= G^n_*\circ f_*\circ (G^n_*)^{-1}$.
\end{enumerate}
Moreover,
\begin{enumerate}
\item [\rm (3)]
$
u_*\circ f_*=f^*\circ u_*.
$
\end{enumerate}
\end{lem}

Along with $u_*$, consider its rescaling 
% Introduce the function $v_*$ defined on $[-1,1]$ given by
$$
v_*: [-1,1]\ra \R, \quad v_*(x)=\frac{1}{u'_*(1)}(u_*(x)-1)+1,
$$
normalized so that $v_*(1)=1$ and $\displaystyle \frac{d v_*}{dx} (1)=1$.

\bigskip

The following Lemma is an improvement of Lemma 7.3 in \cite{CLM}. Although the proof of this Lemma is essentially the same, we include it here with the small change.

\begin{lem}\label{convergence to g-star}
  Let $\rho\in (0,1)$, $C>0$.  
Consider a sequence of smooth functions $g_l: [-1,1]\ra [-1,1]$, $l=1,\dots, n$,
 such that 
$\| g_k - g_*\|_{C^3}\leq C \rho^l$. Let
$g^n_k=g_k\circ\dots\circ g_n$, 
and let         
$G^n_k= a^n_k\circ g^n_k: [-1,1]\ra [-1,1]$, where $a^n_k$ is the affine rescaling of 
$\Im g^n_k$
 to $[-1,1]$. 
Then  
$$
\|G^n_k - G_*^{n-k+1}\|_{C^2}\leq C_1 \rho^{\frac{n}{2}},
$$
 where $C_1$ depends only 
on $\rho$ and $C$.
\end{lem}   
 
\begin{proof}   
Let $I_0=[-1,1]$ and $I_j=[x_j,y_j]\subset [-1,1]$ such that 
$g_{n-j}(I_j)=I_{j+1}$. 
Rescale affinely the domain and image of $g_{n-j}\colon I_j\to I_{j+1}$
and denote the normalized diffeomorphism by $h_{n-j}\colon [-1,1]\to [-1,1]$.
Let
$$
I_j^*=[x_j^*,1]=g_*^{j}([-1,1])
$$
and rescale the domain and image of $g_*\colon  I_j^*\to I_{j+1}^*$ and
denote the normalized diffeomorphism by $h_{n-j}^*\colon [-1,1]\to
[-1,1]$. Note that
$$
h_{k}^*\circ h_{k+1}^*\circ \cdots \circ h_n^* \to
u_*,
$$
where the convergence in the $C^2$ topology is exponential in $n-k$. 
In the following estimates we 
will use a uniform constant $\rho<1$
for exponential estimates.
Let $\Delta x_j=x_j-x^*_j$ and $\Delta y_j= y_j-1$  . Use, $g_{n-j}(x_j)=x_{j+1}$,
then
$$
x_{j+1}=g_*(x^*_j)+g_*'(\zeta_j) \cdot \Delta x_j +O(\rho^{n-j}).
$$
We may assume that the maximal derivative of $g_*$ is smaller than $\rho<1$. 
Then
$$
\begin{aligned}
\Delta x_j&\le \sum_{l=0}^{j-1} C\rho^{n-l} \prod_{k=l+1}^{j-1} g_*'(\zeta_k)\\
&\le C \sum_{l=0}^{j-1} \rho^{n-l} \rho^{j-1-l}\\
&= C \rho^{n-j+1} \sum_{l=0}^{j-1} (\rho^2)^{j-l-1}\\
&=O(\rho^{n-j}).
\end{aligned}
$$
Use a similar argument for  $\Delta y_j$ to get
\begin{equation}\label{xy}
|\Delta x_j|, |\Delta y_j|= O(\rho^{n-j}).
\end{equation}
Because, $g_l$ and $g_*$ are contractions we have
\begin{equation}\label{II*}
|I_j|, |I^*_j|=O(\rho^{j}).
\end{equation}
We will represent a diffeomorphism  $\phi:I\to J$ by its nonlinearity
\begin{equation}\label{nonl}
\eta_\phi=\frac{D^2\phi}{D\phi}.
\end{equation}
The use of the nonlinearity is that it allows to control distortion
\begin{equation}\label{intnonl}
\log \frac{D\phi(y)}{D\phi(x)}=\int_x^y \eta.
\end{equation}
Let $\eta_l$ and $\eta^*$ be the nonlinearities of $g_l$ and $g_*$.
Notice that
$$
\|\eta_l-\eta^*\|_{C^1}=O(\rho^l).
$$
Furthermore, let  $\mathbb{I}_j:[-1,1]\to I_j$ and 
$\mathbb{I}^*_j:[-1,1]\to I^*_j$
be the affine orientation preserving rescalings. Using this notation 
$$
\eta_{n-j}(\mathbb{I}_j(x))=\eta^*(\mathbb{I}^*_j(x))+
D\eta^*(\zeta_j)\cdot \left(\mathbb{I}_j(x)-\mathbb{I}^*_j(x)\right)+  O(\rho^{n-j}),
$$
for some $\zeta_j\in [\mathbb{I}_j(x),\mathbb{I}^*_j(x)]$.
Hence,
$$
\eta_{n-j}(\mathbb{I}_j(x))=\eta^*(\mathbb{I}^*_j(x))+
     O(\rho^{n-j}).
$$
The nonlinearities of $h_{n-j}$ and $h^*_{n-j}$ are given by
\begin{equation}\label{etaj}
\eta_{h_{n-j}}=|I_j|\cdot \eta_{n-j}(\mathbb{I}_j),
\end{equation}
and similarly
\begin{equation}\label{eta*j}
\eta_{h^*_{n-j}}=|I^*_j|\cdot \eta^*(\mathbb{I}^*_j).
\end{equation}
Now,
$$
\begin{aligned}
|\eta_{h_{n-j}}(x)-\eta_{h^*_{n-j}}(x)|&=
O((|I_j|-|I^*_j|)+ \rho^{n-j}\cdot |I^*_j|)\\
&=O((|I_j|-|I^*_j|)+\rho^n).
\end{aligned}
$$
Use (\ref{xy}) and (\ref{II*}) 
$$
|\eta_{h_{n-j}}(x)-\eta_{h^*_{n-j}}(x)| =
\left\{
\begin{array}{ccc }
O(\rho^{n-j}) & : & j\leq n/2 
\\ 
O(\rho^{j}) & : & n-k+1\ge j> n/2.
\end{array} \right.
$$
It follows that
$$
\sum_{j=0}^{n-k+1} \|\eta_{h_{n-j}}- \eta_{h^*_{n-j}}\|_{C^0}=O(\rho^{\frac{n}{2}}).
$$
Note that we can estimate $\|\eta_{h_{n-j}}\|_{C^1}$ by using
$$
D\eta_{h_{n-j}}=|I_j|^2 D\eta_{n-j}(\mathbb{I}_j).
$$
This and (\ref{etaj}), (\ref{eta*j}) give a universal bound on 
$\sum_{j=0}^{n-k+1} \|D\eta_{h^{(*)}_{n-j}}\|_{C^1}$.
These bounds, allow use to use
a reshuffling argument,   
see \cite[Lemma 14.1]{CLM},  which finishes the
proof of the Lemma.
\end{proof}
}
The renormalization fixed point $f_*$ has a nested sequence of renormalization cycles $\CC_n$, $n\ge 1$. A cycle consists of the following intervals. The critical point of $f_*$ is $c_*$ and the critical value $v_*=f_*(c_*)$
$$
I^*_j(n)=[f^{j}_*(v_*), f^{j+2^n}_*(v_*)]\in \CC_n,
$$
with $j=0,1,2, \cdots, 2^n-1$. The collection $\CC_n$ consists of pairwise disjoint intervals. Notice, for  $j=0,1,2,\dots, 2^n-2$
$$
f_*(I^*_j(n))=I^*_{j+1}(n),
$$
and
$$
f_*(I^*_{2^n-1}(n))=I^*_0(n).
$$
The interval in $\CC_n$ which contains the critical point is denoted by
$$
U_n=I^*_{2^n-1}(n)\ni c_*.
$$

\bigskip

The {\it nonlinearity} of a $C^2$-diffeomorphism $\phi:I\to \phi(I)\subset \Bbb{R}$, $I\subset \Bbb{R}$, is
\begin{equation}\label{nonlin}
\eta_{\phi}=D\ln D\phi.
\end{equation}
The {\it Distortion} of a diffeomorphism $\phi:I\to J$ between intervals $I,J\subset \Bbb{R}$ is defined as
$$
\text{Dist}(\phi)=\max_{x,y}\log \frac{D\phi(y)}{D\phi(x)}.
$$
If $\eta$ is the nonlinearity of $\phi$ then
\begin{equation}\label{distnonl}
\text{Dist}(\phi)\le \|\eta\|_{C^0}\cdot |I|.
\end{equation}
The distortion of a map does not change if we rescale domain and range.




Given $r>0$. The $r$-neighborhood $T\supset I$ of an interval $I\subset \Bbb{R}$ is the interval such that both components of $T\setminus I$ have length $r|I|$. 

\begin{lem}\label{distortion}  There exist $r>0$ and $D>1$ such that the $r$-neighborhoods $T_j(n)\supset I^*_j(n)$ have the following property. For all $n\ge 1$ the following holds. Let $\zeta_j\in T_j(n)$ then
$$
\prod_{l=k_1}^{k_2-1}\frac{|Df_*(\zeta_j)|}{\frac{|I^*_{j+1}(n)|}{|I^*_j(n)|}}\le D.
$$
with $0\le k_1<k_2<2^n$.
\end{lem}

\begin{proof} The a priori bounds on the cycles $\CC_n$ are described in \cite{MS}, see also
\cite{CMMT}. The a priori bounds state that for some $r>0$ the gap between $I_j(n+1)$ and $I_{j+2^{n+1}}(n)$ satisfies
$$
|I_j(n)\setminus (I_j(n+1)\cup I_{j+2^{n+1}}(n))|\ge 5r\cdot  |I_j(n)|.
$$
Hence, we have  
$T_j(n+1)\cap T_{j+2^{n+1}}(n+1)=\emptyset$ and 
$$
|T_j(n+1)|+|T_{j+2^{n+1}}(n)|\le (1-r)\cdot  |T_j(n)|.
$$
Let $\eta_j(n)$ be the nonlinearity, see (\ref{nonlin}), of the rescaling of $f_*:I^*_j(n)\to I^*_{j+1}(n)$. The rescaling turns domain and range into $[-1,1]$.
Lemma 3.1 in \cite{Ma2} says that
$$
\begin{aligned}
\|\eta_j(n+1)\|_{C_0}&\le \frac{|T_j(n+1)|}{ |T_j(n)|}\cdot \|\eta_j(n)\|_{C_0}, \\
\|\eta_{j+2^{n+1}}(n+1)\|_{C^0}&\le \frac{|T_{j+2^{n+1}}(n+1)|}{ |T_j(n)|}\cdot \|\eta_j(n)\|_{C_0}.
\end{aligned}
$$
Hence, 
$$
\|\eta_j(n+1)\|_{C_0}+\|\eta_{j+2^{n+1}}(n+1)\|_{C^0}\le (1-r)\cdot \|\eta_j(n)\|_{C_0},
$$
for $j=0,1,2,\cdots, 2^{n}-2$.
The a priori bounds also imply a universal bound 
$$
\|\eta_{2^n-1}(n+1)\|_{C_0}\le K.
$$
Inductively, this gives a universal bound
$$
\sum_{j=0}^{2^n-2} \|\eta_{j}(n)\|_{C_0}\le K_0.
$$
Use (\ref{distnonl}) and observe,
$$
\log \frac{|Df_*(\zeta_j)|}{\frac{|I^*_{j+1}(n)|}{|I^*_j(n)|}}=O(\|\eta_j(n)\|_{C_0}).
$$
The Lemma follows.
\end{proof}


\begin{prop}\label{disto} There exists $\rho<1$ such that the following holds. Let  $0<q_0$ and 
$I\in \CC_n$ and $I\subset U_{k}\setminus U_{(1-q_0)\cdot n}$, with $k<(1-q_0)\cdot n$. Let $t_I=2^{k}$ be the first return to 
$U_{k}$. Then for every $j\le t_I$
$$
\text{Dist}(f_*^j|I)=O(\rho^{q_0\cdot n}).
$$
\end{prop}

\begin{proof} Let $s_I\ge t_I$ be the first return time of $I$ to $U_{(1-q_0)\cdot n}$. There exists $J_0\subset U_{k}$ with $I\subset J_0$ such that
$f_*^{s_I}: J_0 \to U_{(1-q_0)\cdot n}$ diffeomorphically, \cite {Ma1}. Let $J_k=f_*^k(J_0)$ and $I_k=f_*^k(I)$. The {\it a priori} bounds on the geometry of the cycles $\CC_n$ imply
$$
\frac{|I_k|}{|J_k|}=O(\rho^{q_0\cdot n}).
$$
This estimate hold because the intervals $J_k$ are in $\CC_{(1-q_0)\cdot n}$ and the intervals $I_k$ are in $\CC_n$. 


The nonlinearity of the rescaled map $f_*:J_k\to J_{k+1}$ which has the unit interval as its domain and range, is denoted by $\eta_k$. As in the proof of Lemma \ref{distortion} we obtain
$$
\sum_{k=0}^{s_I-1} \|\eta_k\|_{C^0}\le K_0.
$$ 
The nonlinearity of the rescaled version of the map $f_*:I_k\to I_{k+1}$ which has the unit interval as its domain and range, is denoted by $\eta^I_k$. Lemma 3.1 in \cite{Ma2} says that the nonlinearity of the restriction $f_*:I_k\to I_{k+1}$ of  $f_*:J_k\to J_{k+1}$ satisfies
$$
\|\eta^I_k\|_{C^0}\le \frac{|I_k|}{|J_k|}\cdot \|\eta_k\|_{C^0}.
$$
Hence,
$$
\sum_{k=0}^{s_I-1} \|\eta^I_k\|_{C^0}=O(\rho^{q_0\cdot n}).
$$ 
The distortion of a map $f_*^t:I_k\to I_{k+t}$ is bounded as follows.
$$
\begin{aligned}
\text{Dist}(f^s_*|I_k)&\le \sum_{j=k}^{k+t-1} \text{Dist}(f_*|I_{j})\\
&\le \sum_{j=0}^{s_I-1} \|\eta^I_j\|_{C^0}=O(\rho^{q_0\cdot n}).
\end{aligned}
$$
This finishes the proof of the Lemma.
\end{proof}



\subsection{Geometrical properties of the Cantor attractor}

\begin{thm}[Universality]\label{universality}
For any $F\in \II_\Om(\bar\eps)$ with sufficiently small $\bar\eps$, we have: 
\[
    R^n F = (f_n(x) -\,  b^{2^n}\, a(x)\, y\, (1+ O(\rho^n)), \ x\, ),
\]
where $f_n\to f_*$ exponentially fast, $b$ is the average Jacobian, $\rho\in (0,1)$,
and $a(x)$ is a universal  function. Moreover, $a$ is analytic and 
positive.   
\end{thm}


\begin{cor}\label{bdsFx} There exists  a universal $d_1>0$ such that for $k\ge 1$ large enough \
$$
 \frac{1}{d_1}\le |\frac{\partial F_k}{\partial x}(z)|\le d_1,
$$
for every $z\in B^1_v(F_k)$.
\end{cor}







Let $\tau_n$ be the tip of $F_n=R^nF$ and $\tau^*$ be the tip of $F_*$. 



\begin{lem}\label{holmt} There exists $\rho<1$ such the 
conjugations
$$
h_n:\OO_{F_*}\to \OO_{F_n}
$$
with $h_n(\tau_*)=\tau_{n}$ satisfy 
$$
|h_n(z)-z|=O(\rho^n),
$$
for every $z\in \OO_{F_*}$.
\end{lem}

\begin{proof} Choose $z^*\in \OO_{F_*}$ and let $z=h_n(z^*)$. There are unique sequence $w_{n+1},\dots, w_m, \dots$, and $z_n, z_{n+1},\dots, z_m,\dots$, and
$z^*_n,z^*_{n+1},\dots, z^*_m,\dots$ with $w_k\in \{c,v\}$, $z_k\in \OO_{F_k}$, and $z^*_k\in \OO_{F_*}$ such that $z=z_n$, $z^*=z^*_n$ and for $k\ge n$
$$ 
z_k=\psi^{k+1}_{w_{k+1}}(z_{k+1})   
$$
$$ 
z^*_k=(\psi^{k+1}_{w_{k+1}})^*(z^*_{k+1}).   
$$
This follows from the construction of $\OO_F$ in \cite{CLM}. 

Theorem \ref{universality} implies
$$
|\psi^{k+1}_w-(\psi^{k+1}_w)^*|=O(\rho^k)
$$
for some $\rho<1$. The proof of Lemma 5.6 in \cite{CLM} gives that
$(\psi^{k+1}_w)^*=\psi^*_w$ are contractions, $|D\psi^*_w|\le \sigma<1$. Then for $k\ge n$
$$
\begin{aligned}
|z_k-z^*_k|=&|\psi^{k+1}_{w_{k+1}}(z_{k+1})-(\psi^{k+1}_{w_{k+1}})^*(z^*_{k+1})|\\
\le &|\psi^{k+1}_{w_{k+1}}(z_{k+1})-(\psi^{k+1}_{w_{k+1}})^*(z_{k+1})|+\\
&|(\psi^{k+1}_{w_{k+1}})^*(z_{k+1})-(\psi^{k+1}_{w_{k+1}})^*(z^*_{k+1})|\\
\le &O(\rho^k)+\sigma\cdot |z_{k+1}-z^*_{k+1}|
\end{aligned}
$$
Then for every $m>n$ we have
$$
|z_n-z^*_n|\le \sum_{k=n+1}^m O(\rho^k)\cdot \sigma^{k-n-1}+\sigma^{m-n}\cdot |z_m-z^*_m|.
$$
Observe, $|z_m-z^*_m|\le 1$ and the Lemma follows by taking $m>n$ sufficiently large.
\end{proof}

\comment{
\begin{cor}\label{tipdist} There exists $\rho<1$ such that for $\Omega$ there exists $C>0$ such that  
$F\in \HH_\Omega$ 
$$
|\tau_n-\tau^*|\le C |F_n-F_*|_{C^2}=O(\rho^n).
$$
\end{cor}

\note{If we don't use the $C^2$ estimate we can skip the proof, it is a cor of Lemma 2.6}
}

\comment{

\begin{proof} The proof is by collecting facts from \cite{LM}. The following notation is illustrated in Figure 7.1 from \cite{LM}. Given $n\ge 1$ denote the graph of $f_n$, see Theorem \ref{universality}, over the $y$-axis by $\Gamma_0$. The map $F_n$ has two fixed points $\beta_0$ and $\beta_1$, where $\beta_1$ has two negative exponents. The local stable manifold of $\beta_1$ is a graph over the $y$-axis very close to a vertical line. Let $\Gamma_2$ be the curve between the first two intersections of the local unstable manifold of $\beta_0$ and $\Gamma_\infty$ be the curve between the first two intersections of the local unstable manifold of $\beta_2$. The curves $\Gamma_0$, $\Gamma_2$, and $\Gamma_\infty$ can be extended to graphs of functions defined on the same domain in the $y$-axis.  
Corollary 7.2 from \cite{LM} states 
$$
|\Gamma_2-\Gamma_\infty|_{C^2}=O(b^{2^n}).
$$
Proposition 7.1(7.1) from \cite{LM} gives
$$
|\Gamma_0-\Gamma_\infty|_{C^2}=O(b^{2^n}).
$$
Hence, 
$$
|\Gamma_0-\Gamma_2|_{C^2}=O(b^{2^n})
$$
and
$$
|v_0-v_2|=O(b^{2^n}),
$$
where $v_0$ and $v_2$ are the points on $\Gamma_0$, $\Gamma_2$ with a vertical tangency. 
Proposition 7.4(3) from \cite{LM} gives
$$
|\tau_n-v_2|=O(b^{2^n}).
$$
Hence,
$$
|\tau_n-v_0|=O(b^{2^n}).
$$
Observe, $|v_0-\tau^*|=O(F_n-F_*)$ and the Lemma follows.
\end{proof}

}

\subsection{Analytical properties of the coordinate changes}


Fix an infinitely renormalizable H\'enon-like map $F\in \II_\Om(\bar\eps)$ 
to which we can apply the results of \cite{CLM} and \cite{LM1}, $\bar\eps>0$ is small enough. For such an $F$, we have a well defined {\it tip}: 
$$
\tau\equiv \tau(F)=\bigcap_{n\ge 0} B^n_{v^n}
$$
Consider the tips of the renormalizations, $\tau_k=\tau(R^k F)$.
To simplify the notations, we will translate these tips to the origin
by letting
$$
 \Psi_k =  \psi^0_v (R^k F)\,  (z + \tau_{k+1}) - \tau_k.  
$$ 
Denote the derivative of the maps $\Psi_k $ at $0$ by $D_k$
and decompose it into the unipotent and diagonal factors: 
 \begin{equation}\label{Dk}
 D_k= \left(
\begin{array}{cc}
1 & t_k\\
0 & 1
\end{array}\right)
\left(
\begin{array}{cc}
\alpha_k & 0\\
0 & \beta_k
\end{array}\right). 
% =\left(
% \begin{array}{cc}
% \alpha_k & \beta_k\cdot t_k\\
% 0 & \beta_k
% \end{array}\right).
\end{equation}
Let us factor this derivative out from $\Psi_k$: 
$$
\Psi_k = D_k \circ (\id + {\bf s}_k),
% \left(
% \begin{array}{c}
% x+ s^k \\
% y
%\end{array}\right)
$$
where ${\bf s}_k(z) = (s_k(z) , 0) =  O(|z|^2)$ near 0.
Lemma 7.4 in \cite{CLM} states


\begin{lem} \label{smalls}
There exists $\rho<1$ such that for $k\in \Z_+$ the following estimates hold:
\begin{enumerate}
% \item $s_k(0,0)=0,$

% \item $\frac{\partial s_k(0,0)}{\partial x}= \frac{\partial s_k(0,0)}{\partial y}=0,$

\item [\rm (1)] $\displaystyle 
  \alpha_k=\sigma^2 \cdot (1+O(\rho^k)),\quad \beta_k=-\sigma \cdot (1+O(\rho^k)), \quad
         t_k=O(\bar\eps^{2^k}); 
$

\item [\rm (2)]
$\displaystyle | \di_x s_k | = O(1),\quad  |\di_y s_k| = O(\bar\eps^{2^k}); $  

\item[\rm (3)]
$\displaystyle
  |\partial^2_{xx} s_k |= O(1),\quad
  |\partial^2_{xy} s_k |= O(\bar{\eps}^{2^k}) ,\quad 
  |\partial^2_{yy} s_k| =O(\bar{\eps}^{2^k}).
$
\end{enumerate}

\end{lem}

\begin{lem}\label{tilt} The numbers $t_k$ quantifying the tilt satisfy$$
t_k\asymp  -b_F^{2^k}.
$$
\end{lem}




We will use the following notation
$$
B^{n-k}_{v^{n-k}}(F_k)=\Im \Psi_k^n.
$$
\comment{
The following statements is Corollary 7.5 from \cite{CLM}

\begin{cor}\label{second derivatives} 
 Let $k<n$. For $z \in B_{v^{n-k}}^{n-k}$ we have: 
% \begin{enumerate}
$$
\left| \partial_x s_k(z)\right|   =O (\sigma^{n-k}), \quad 
\left| \partial_y s_k(z)  \right| =
      O(\bar{\eps}^{2^k}\cdot\sigma^{n-k}).
$$
%\end{enumerate}
\end{cor}

\note{did we use this Cor?}
}
Consider the derivatives of the maps $\Psi^n_k$ at the origin:  
$$
D_k^n=D_k\circ D_{k+1}\circ \cdots D_{n-1}.
$$
We can reshuffle this composition and obtain:

 \begin{equation}\label{reshuffling}
 D_k^n= 
 \left(
\begin{array}{cc}
1 & t_k\\
0 & 1
\end{array}\right)
\left(
\begin{array}{cc}
(\si^2)^{n-k} & 0\\
0 & (-\si)^{n-k}
\end{array}\right) (1+O(\rho^k)). 
\end{equation}  
%
%
Factoring the derivatives  $D_k^n$ out from $\Psi_k^n$, we obtain: %  a representation
\begin{equation}\label{factoring}
\Psi_k^n = D_k^n \circ (\id + {\bf S}_k^n),
%\left(
%\begin{array}{c}
%x+S_n^k\\
%y
%\end{array}\right).
\end{equation}
where ${\bf S}_k^n (z) = (S_k^n(z), 0) = O(|z|^2)$ near 0. 

The following Lemma is Lemma 7.6 in \cite{CLM}

\begin{lem}\label{APPsi} For $k<n$,  we have:
\begin{enumerate}

\item [{\rm (1)}]
$ \displaystyle
   | \di_x S^n_k | = O(1),\quad  |\di_y S^n_k | = O(\bar{\eps}^{2^k}); 
$

\item [{\rm (2)}]
$ \displaystyle
|\partial^2_{xx} S^n_k| =O(1), \quad
|\partial^2_{yy} S^n_k| =O(\bar{\eps}^{2^k}), \quad
|\partial^2_{xy} S^n_k| =O(\bar{\eps}^{2^k}\, \si^{n-k}).
$
\end{enumerate}


\end{lem}



\begin{lem}\label{bdsS'} There exists  a universal $d_0>0$ such that for $k\ge 1$ large enough \
$$
 \frac{1}{d_0}\le |\frac{\partial(\id + {\bf S}_k^n)}{\partial x}|\le d_0
$$
\end{lem}

\begin{proof} According to proposition 7.8 in \cite{CLM}, the diffeomorphisms 
$\id + {\bf S}_k^n$ stay wihin a compact family of diffeomorphisms. This gives the upperbound on 
the derivative. The partial derivative $\frac{\partial(\id + {\bf S}_k^n)}{\partial x}$ can not be zero in a point because otherwise the derivative of the diffeomorphism  would become singular in point. This gives the positive lower bound on the partial derivative. 
\end{proof}



\comment{

We are now ready to describe the asymptotical behavior of the $\Psi$-functions
using the universal one-dimensional functions from  \S \ref{1D universal f-s}. 
Let us normalize the function $v_*$ so that it fixes $0$ rather than $1$: 
$$
   {\bf v}_*(x) = v_*(x+1)-1.
$$ 


\begin{lem}\label{ustar}
 There exists $\rho<1$ such that  for all $k<n$ and $y\in I$,
$$
\left|\id +  S^n_k (\cdot,y)-{\bf v}_*(\cdot)\right|=O(\bar{\epsilon}^{2^k}\cdot y+
\rho^{n-k})
$$
and
$$
  \left| 1+ \frac{\partial S_k^n}{\partial x}(\cdot,y)-
\frac{\partial {\bf v}_*}{\partial x}(\cdot)\right|=O(\rho^{n-k}).
$$
\end{lem}


\begin{prop}\label{limit}
 There exists a coefficient $a_k\in \mathbb{R}$, $a_k=O(b^{2^k})$ and an absolute constant $\rho\in (0,1)$ such that 
$$
\left|(x + S^l_k(x,y))-({\bf v}_*(x)+a_k y^2)\right|=O(\rho^{l-k}).
$$
\end{prop}

\begin{proof} By  Lemma \ref{APPsi}, 
$$
\left|\frac{\partial^2 S_k^n}{\partial yx} \right|=O(\bar\eps^{2^k}\sigma^{n-k})=O(\sigma^{n-k})
$$
and
$$
\left|\frac{\partial S_k^n}{\partial y} \right|=O(\bar{\epsilon}^{2^k}).
$$
Hence it is enough to verify the desired convergence on the horizontal section passing through the tip: 
$$
\dist_{C^1}(\id + S_k^n (\cdot, 0 ),\, {\bf v}_*(\cdot))=O(\rho^{n-k}).
$$ 


% Let $g_k(x)= \Psi_k(x-1,0)+1: I\ra I$.
Let us normalize $g_*$ so that $0$ becomes its fixed point with $1$ as 
multiplier:   
$$  
          \Bg_*(x) = \frac{g_*(x+1)-1}{g_*'(1)}.
$$   
Now, $\id+S^n_k(\cdot, 0)$ is the rescaling of $\Psi^n_k(\cdot, 0)$ 
normalized so 
that
the fixed point $0$ has  multiplier 1. By Theorem 4.1, 
$$
    \dist_{C^3}(\id+ s_k(\cdot, 0), \Bg_*(\cdot)) = O(\rho^k).
$$
Hence, by  Lemma \ref{convergence to g-star},  
$$
    \dist_{C^1}(\id + S^n_k(\cdot,0), \Bg_*^{n-k}(\cdot)) = O(\rho^{k}) .
$$ 
Since $\Bg^n \to {\bf v}_*$ exponentially fast, the conclusion follows. 
\end{proof}


Let $(S^n_k)^*(x,y)=v_*(x)-x$ be the non affine part of the coordinate changes used to renormaliza $F_*$. 



\begin{prop}\label{limit}
 There exists  an absolute constant $\rho\in (0,1)$ such that 
$$
\left|(x + S^n_k(x,y))-(x+(S^n_k)^*(x))\right|=O(\rho^{n},\rho^{n-k}+b^{2^k}\cdot y^2\}), 
$$
with $n>k$.
\end{prop}

The proof is the same as the proof of Proposition 7.8 in \cite{CLM} together with the observation that 
$$
a_F=O(b^{2^k})
$$
when applied to $S^n_k$.

\begin{proof} The image  of the vertical interval  $y\mapsto (0,y)$
under the map $\id + \BS_0^n$ is the graph of a function $w_n:I\to \mathbb{R}$ defined by
$$
w_n(y)=S_0^n(0,y).
$$
By the second part of  Lemma~\ref{ustar} we have: 
$$
\left|(x + S^n_0(x,y))-({\bf v}_*(x) + w_n(y) )\right|
=O(\rho^n).
$$
Let us show that the functions $w_n$ converge to a parabola. 
The identity
$$
   D_0^{n+1}\circ (\id + \BS^{n+1}_0) = \Psi^{n+1}_0=\Psi^n_0\circ \Psi_n= D^n_0\circ(\id +\BS^n_0)\circ D_n\circ (\id+{\bf s}_n),
$$
implies
$$
   \BS^{n+1}_0= {\bf s}_n+ D_n^{-1}\circ \BS^n_0\circ D_n\circ (\id+{\bf S}_n),
$$
so that
\begin{equation}\label{w sub n}
w_{n+1}(y)=s_n(0,y)+ \frac{1}{\alpha_n} S_0^n(\alpha_n s_n(0,y)+\beta_n t_n y,\, \beta_n y),
\end{equation}
where $\alpha_n, \beta_n$ and $t_k$ are the entries of $D_n$, see 
equation~(\ref{Dk}).
The estimate of $\di_y s_n$ from  Lemma \ref{smalls} implies:
\begin{equation}\label{s sub n}
s_n(0,y)=e_n y^2 + O(\bar\eps^{2^n} y^3),
\end{equation}
where $e_n=O(\bar{\epsilon}^{2^n})$.
% and $\|K_s\|=O(\bar{\epsilon}^{2^n})$.
%The Taylor expansion of $S_0^n$ begins with only quadratic terms. This implies
The estimate of $\di_{xy}^2 S^n_0$ from Lemma \ref {APPsi} implies:
$$
  \frac{\di S_0^n}{\di x}(0,y) = O(\bar\eps^{2^n} y).
$$
Hence
$$
S_0^n(\alpha_n s_n(0,y)+\beta_n t_n y,\, \beta_n y)
$$
$$
= S^n_0(0,\beta_n y)+ 
      \frac{\di S^n_0}{\di x} (0, \beta_n y) (\alpha_n s_n(0,y)+\beta_n t_n y)+O(\bar\eps^{2^n} y^3)
$$
$$
   = S^n_0(0, \beta_n y) + q_n y^2 + O(\bar\eps^{2^n} y^3 )= w_n(\beta_n y) + q_n y^2 + O(\bar\eps^{2^n} y^3 ),
$$
where $q_n= O(\bar\eps^{2^n})$.
Incorporating this and (\ref{s sub n}) into (\ref{w sub n}), we obtain: 
$$
w_{n+1}(y)= \frac{1}{\alpha_n} w_n(\beta_n y)+
             c_n y^2 + O(\bar\eps^{2^n} y^3),
$$
where $c_n=O(\bar{\epsilon}^{2^n})$. % and $\|C_n\|=O(\bar{\epsilon}^{2^n})$.
% Hence
% $$
% w_{n+1}(y)= \frac{1}{\alpha_n} w_n(\beta_n y) + p_n y^2 +P_n(y) y^3,
% $$
% with $p_n=O(\bar{\epsilon}^{2^n})$ and $\|P_n\|=O(\bar{\epsilon}^{2^n})$.
% Introduce $a_n$ and $A_n(y)$ such that
Writing $w_n$ in the form
$$
w_n(y)=a_ny^2 +A_n(y) y^3, 
$$
we obtain: 
$$
a_{n+1}=\frac{\beta_n^2}{\alpha_n} a_n +c_n
$$
and
$$
\|A_{n+1}\|\le \frac{|\beta_n|^3}{\alpha_n}\|A_n\|+ O(\bar\eps^{2^n}).
$$
Now  the first item of Lemma~\ref{smalls} 
% use $\alpha_n=\sigma^2 \cdot (1+\rho^n)$ and $\beta_n=\sigma\cdot (1+\rho^n)$ and the exponential convergence of 
implies that $a_n\to a_F$ and $\|A_n\|\to 0$ exponentially fast.
\end{proof}

}

\begin{lem}\label{deltapsi} There exists $\rho<1$ such that
$$
|\Psi^n_k-(\Psi_k^n)^*|_{C^0}=O(\rho^k).
$$
\end{lem}

\begin{proof} The proof is a small modification of the proof of 
Lemma \ref{holmt}. Use the same notation: $w_l=v$ for all $l\ge k$.
We have to incorporate the translation which center the maps around the tips.
The estimates in the proof of Lemma \ref{holmt} become
$$
|\Psi^n_k(z)-(\Psi_k^n)^*(z)|
\le O(\rho^k)+\sum_{l=k+1}^n O(\rho^l)\cdot \sigma^{l-k-1}+\sigma^{n-k}\cdot |z_n-z^*_n|,
$$
where $z_n=z+\tau_n$ and $z^*_n=z+\tau^*$.  From Lemma \ref{holmt} we get that
$|z_n-z^*_n|=O(\rho^n)$ and the Lemma follows.
\end{proof}








\subsection{General Notions}

We will use the following general notions and notations throughout the text.

Let $\subset \Bbb{R}^2$ and $Q=[a,a+h]\times [b,b+v]$ be the smallest rectangle containing $X$. Then $h\ge 0$ is the horizontal size of $X$ and $v\ge 0$ the vertical size.

$Q_1\asymp Q_2$ means that $C^{-1}\le Q_1/Q_2\le C$, where $C>0$ is 
an absolute constant or depending on, say $F$. Similarly, we will use $Q_1\gtrsim Q_2$.







